How Concise are Chains of co-B\"uchi Automata?

Chains of co-B\"uchi automata (COCOA) have recently been introduced as a new canonical model for representing arbitrary omega-regular languages. They can be minimized in polynomial time and are hence an attractive language representation for applications in which normally, deterministic omega-automata are used. While it is known how to build COCOA from deterministic parity automata, little is currently known about their relationship to automaton models introduced earlier than COCOA. In this paper, we analyze the conciseness of chains of co-B\"uchi automata. We show that even in the case that all automata in the chain are deterministic, chains of co-B\"uchi automata can be exponentially more concise than deterministic parity automata. We then answer the question if this conciseness is retained when performing Boolean operations (such as disjunction and conjunction) over COCOA by showing that there exist families of languages for which these operations lead to an exponential growth of the sizes of the automata. The families have the property that when representing them using deterministic parity automata, taking the disjunction or conjunction of them only requires a polynomial blow-up, which shows that Boolean operations over COCOA do not retain their conciseness in general.

==> eptcsdata.tex <==
\providecommand{\firstpage}{111}
\providecommand{\publicationstatus}{G. Bacci, A. Francalanza (Eds.): Sixteenth\\ International Symposium on Games, Automata, Logics,\\ and Formal Verification (GandALF 2025)\\
EPTCS 428, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.428.9}{10.4204/EPTCS.428.9}}

